An Integer Linear Programming Model for Tilings

In this paper, we propose an Integer Linear Model whose solutions are the aperiodic rhythms tiling with a given rhythm A. We show how this model can be used to efficiently check the necessity of the Coven-Meyerowitz's $(T2)$ condition and also to define an iterative algorithm that finds all the possible tilings of the rhythm A. To conclude, we run several experiments to validate the time efficiency of this model.

==> scarti.tex <==
\subsubsection*{Aperiodicity }

% Our aim is to find rhythms $B$, where $B$ is required to be \textit{aperiodic}.
%
Suppose that $n = p_1^{\alpha_1} p_2^{\alpha_2} \dots p_N^{\alpha_N}$ is the complete and unique factorization of $n$ in distinct primes. 
%
By Remark \ref{aperiodic}, it is enough to check the aperiodicity conditions only for certain ``maximal" periods. For this reason, we introduce the following definition.
%
\begin{definition}
Let $p_i$ be a prime divisor $n$, then we call a maximal product of $n$ the natural number
\[
m_i=\frac{n}{p_i} \quad\quad\quad \text{where }\quad p_i\in \Pn
\]
where $\Pn $ denotes the set of all primes $p_i \in Div(n)$, where $Div(n)$ is the set of divisors of $n$. We denote with $\mathcal{M}_n$ the set containing all the maximal product of $n$.
\end{definition}

Let $B = \{b_0, \dots , b_{n_B-1}\}$ be a rhythm and $m_k \in \mathcal{M}_n$ be a maximal product.

If $B$ is aperiodic with \greta{questo lo toglierei: (respect to the period $m_k$)} \genna{ anche il "with" di prima a questo punto, no?}, it satisfies the condition
\[ 
\sum_{j = 0}^{m_k-1 }b_{j} \leq n_B\frac{m_k}{n} -1, \quad \quad \quad \greta{\min} m_k \in \mathcal{M}_n,
\] 
modulo an affine transformation.
%
\noindent Since these conditions are linear, we can add them to the complete Integer Linear Programming model (ILP), in the following form:

\begin{align}
\label{m1:obj}  \min \quad & \sum_{k = 0}^{n-1} x_k \\
\label{m1:c1} \mbox{s.t.} \quad  & \sum_{j=0}^{i} a_{i-j}x_j - r_i = 0 & \forall i\in\{0,\dots,n-1\},\\
\label{m1:c2} & \sum_{j=0}^{i+1} a_{n-(i-j)}x_j - r_{i+n} = 0 & \forall i\in\{0,\dots,n-2\},\\
\label{m1:c3}  &  r_{j}+r_{j+n} =1 & \forall j\in\{0,\dots,n-1\}, \\
\label{m1:c4}  & \sum_{j = 0}^{m_k-1}x_{j} \leq n_B\frac{m_k}{n} -1  & \forall m_k \in \mathcal{M}_n,\\
\label{m1:c5} & x_k,r_k \in \{0,1\} & \forall k \in \{0,\dots,2n-1\}. %\\
%\label{m1:c6} & 
\end{align}


\begin{table}[]
    \centering
\caption{Comparison.\label{Comparison}}
		\begin{tabular}{||c|c|c|c|c|c|c|c ||} 
			\hline
			n &A &number of $B$ according to $E_M$ &number of $ B $ according to $C_M$  & Runtime $E_M$ & Runtime $C_M$\\ [0.5ex] 
			\hline\hline
			72 && 6 (2)  &3 (1) &0.096 &\\
			\hline\hline
			108 &&252 (30)&3 (1) &8.03 &\\
			\hline\hline
			120 &&18 (4)&8  (2) &0.29 &\\
			\hline
			120 &&20 (3)&16 (5) &0.15 &\\
			\hline\hline
			144 &&36 (10)&6 (1) &2.97 &\\
			\hline
			144 && 8640 (591)&3 (1) &&\\
			\hline
			144 &&6 (2)&12 (9) &0.12 &\\
			&&6 (2)&312 (1)&&\\
			\hline
			144&&12 (2)&6 (1)& 0.23 &\\
			 &&48 (7)&6 (1)&&\\
			 &&12 (2)&156 (9)&&\\
			\hline\hline
			168 &&54 (8)&16 (3)& 17.61 &\\
			\hline
			168 &&42 (4)&104 (15)&0.91 &\\
			\hline\hline
			180 &&2052 (136)&8 (2)&&\\
			\hline
			180 &&96 (12)&6 (1)& 48.04 &\\
			\hline
			180 &&$\geq$1800 (171)&16 (5)&466&\\
			\hline
			180 &&120 (18)& 9 (2)& 8.82&\\
			\hline
	\end{tabular}
	
\end{table}


==> tabella.tex <==
\begin{table}[]
    \centering\tiny
\caption{Enumeration Vuza canons.\label{enumvuza}}
		\begin{tabular}{||c| c| c | c| c |c|c|c|c ||} 
			\hline
			$ n $&$ R_{A} $&$ R_{B} $&number of $ A $'s&number of $ B $'s &LP $A$& F-O $A$&LP $B$&F-O $B$\\ [0.5ex] 
			\hline\hline
			72 &$\{2,8,9,18,72\}$&$ \{3,4,6,12,24,36\} $& 6 (2)  &3 (1) &0.096 & 1.59 & 0.02 & 0.33\\
			\hline\hline
			108 &$ \{3,4,12,27,108\} $&$ \{2,6,9,18,36,54\} $&252 (30)&3 (1) &7.84 & 896.06 & 0.03 & 0.72\\
			\hline\hline
			120 &$ \{2,5,8,10,15,30,40,120\} $&$\{3, 4, 6, 12, 20, 24, 60\} $ &18 (4)&8  (2) &0.27 & 24.16 & 0.07 & 2.13\\
			\hline
			120 &$ \{2, 3, 6, 8, 15, 24, 30, 120\} $&$ \{4,5,10,12,20,40,60\} $&20 (3)&16 (5) &0.14 & 10.92 & 0.15 & 3.30\\
			\hline\hline
			144 &$ \{2,8,9,16,18,72,144\} $&$ \{3,4,6,12,24,36,48\} $&36 (10)&6 (1) &2.93 & 82.53  & 0.06 & 3.77\\
			\hline
			144 &$ \{2, 4, 9, 16, 18, 36, 144\} $&$ \{3,6,8,12,24,48,72\} $&8640 (591)&3 (1) &&&&\\
			\hline
			144 &$ \{4, 9, 16, 18, 36, 144\} $&$ \{2, 3, 6, 8, 12,18, 24, 48, 72\} $&6 (2)&12 (9) &0.12 & 7.16 & 1.08 & 37.55 \\
			&\color{lightgray}$ \{4, 9, 16, 18, 36, 144\} $&$ \{2, 3, 6, 8, 12, 24, 48, 72\} $&\color{lightgray}6 (2)&312 (1)&&&&\\
			\hline
			144&$ \{2,9,16,18,36,144\} $&$ \{3, 4, 6, 8, 12, 24, 36,48, 72\} $&12 (2)&6 (1)&0.23 &&&\\
			 & $\{2,9,16,18,144\} $&\color{lightgray}$ \{3, 4, 6, 8, 12, 24, 36,48, 72\} $&48 (7)&\color{lightgray}6 (1)&&&&\\
			 &\color{lightgray}$ \{2,9,16,18,36,144\} $&$ \{3, 4, 6, 8, 12, 24, 48, 72\} $&\color{lightgray}12 (2)&156 (9)& 0.83  & 67.91 & 1.71 & 74.78\\
			\hline\hline
			168 &$ \{2, 7, 8, 14, 21, 42, 56, 168\} $&$ \{3, 4, 6, 12, 24, 28, 84\} $&54 (8)&16 (3)& 17.61 & 461.53 & 0.13 & 7.91\\
			\hline
			168 &$ \{2, 3, 6, 8, 21, 24, 42, 168\}$&$ \{4, 7, 12, 14, 28, 56, 84\} $&42 (4)&104 (15)&0.91 & 46.11 & 1.94 & 35.36\\
			\hline\hline
			180 &$ \{3, 4, 5, 12, 15, 20, 45, 60, 180\} $&$ \{2, 6, 9, 10, 18, 30, 36, 90\} $&2052 (136)&8 (2)&1422 &  & & 0.25\\
			\hline
			180 &$ \{2,5,9,10,18,20,45,90,180\} $&$ \{3, 4, 6, 12, 15, 30, 36, 60\} $&96 (12)&6 (1)& 48.04 & 900.75 & 0.11 & 8.22\\
			\hline
			180 &$ \{3, 4, 9, 12, 36, 45, 180\} $&$ \{2, 5, 6, 10, 15, 18, 20, 30, 60, 90\} $&$\geq$1800 (171)&16 (5)& 503 &&&\\
			\hline
			180 &$ \{2,4,9,18,20,36,180\} $&$ \{3,5,6,10,12,15,30,45,60,90\} $&120 (18)& 9 (2)& 8.82& 280.72 & 0.29 & 14.34\\
			\hline
			% 27225 --> 726.48
	\end{tabular}
	
\end{table}

